Subtitles to Segmentation: Improving Low-Resource Speech-to-Text Translation Pipelines

In this work, we focus on improving ASR output segmentation in the context of low-resource language speech-to-text translation. ASR output segmentation is crucial, as ASR systems segment the input audio using purely acoustic information and are not guaranteed to output sentence-like segments. Since most MT systems expect sentences as input, feeding in longer unsegmented passages can lead to sub-optimal performance. We explore the feasibility of using datasets of subtitles from TV shows and movies to train better ASR segmentation models. We further incorporate part-of-speech (POS) tag and dependency label information (derived from the unsegmented ASR outputs) into our segmentation model. We show that this noisy syntactic information can improve model accuracy. We evaluate our models intrinsically on segmentation quality and extrinsically on downstream MT performance, as well as downstream tasks including cross-lingual information retrieval (CLIR) tasks and human relevance assessments. Our model shows improved performance on downstream tasks for Lithuanian and Bulgarian.

==> eval.tex <==
\begin{table*}[!t]
\label{mqwvltopus}
\centering
\begin{tabular}{ lccc|ccc|ccc }
\toprule
 Model & \multicolumn{3}{c}{EDI-NMT} & \multicolumn{3}{c}{UMD-NMT}  & \multicolumn{3}{c}{UMD-SMT} \\
 & NB & TB & CS & NB & TB & CS & NB & TB & CS\\
\midrule
Acous.  & 0.158 & 0.158 & 0.164 & \textbf{0.230} & \textbf{0.214} & \textbf{0.163} & \textbf{0.263} & \textbf{0.244} & 0.205 \\
 Sub & 0.185 & \textbf{0.178} & 0.193 & 0.185 & 0.203 & 0.113 & 0.255 & 0.223 & \textbf{0.234}  \\
 Sub+S & \textbf{0.191} & 0.170 & \textbf{0.209} & 0.203 & 0.185 & 0.118 & 0.251 & 0.224 & 0.218\\
\bottomrule
\end{tabular}
\caption {AQWV scores on EVAL set for Lithuanian. +S indicates model with syntactic features.}
\label{aqwveval}
\end{table*}

==> full_human.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{ c c ccc }
\toprule
\multirow{2}{*}{Lang.} & \multirow{2}{*}{MT} &  \multicolumn{3}{c}{Relevance}  \\
&   & A & M & R\\
  \midrule
  \multirow{3}{*}{BG} 
 & EDI-NMT &   0.564 & \textbf{0.566} & 0.862\\
 & UMD-NMT &  0.572 &\textbf{0.615} & 0.862\\
   & UMD-SMT & 0.593 &  \textbf{0.658} &0.862\\
   \midrule
\multirow{3}{*}{LT} & EDI-NMT  & \textbf{0.576} & 0.554 & 0.9  \\
 & UMD-NMT  & \textbf{0.663} & 0.593 & 0.9  \\
  & UMD-SMT  & \textbf{0.681} & 0.614 & 0.9 \\
\midrule
\multirow{2}{*}{Lang.} & \multirow{2}{*}{MT} &  \multicolumn{3}{c}{Quality}  \\
&   & A & M & R\\
  \midrule
  \multirow{3}{*}{BG} 
 & EDI-NMT &	\textbf{0.155} &  0.09 & 0.917 \\
 & UMD-NMT & \textbf{0.033} & 0.003 & 0.917 \\
   & UMD-SMT & \textbf{-0.12} & -0.2	& 0.917 \\
   \midrule
\multirow{3}{*}{LT} & EDI-NMT  & \textbf{0.227} & 0.12 & 1.153  \\
 & UMD-NMT  & \textbf{	-0.183} & -0.535 & 1.153 \\
  & UMD-SMT  & \textbf{	-0.45} & -0.591 & 1.153\\
\bottomrule
\end{tabular}
\caption {Human Evaluation comparing relevance and quality using ASR and MT paired with the baseline acoustic segmentation (A), our OpenSubtitles+S model (M),  or
with human reference transcription, segmentation, and translation (R).}
\label{humanresult}
\end{table}

==> tmp.tex <==










